Coverage analysis of information dissemination in throwbox-augmented DTN

This paper uses a bipartite network model to calculate the coverage achieved by a delay-tolerant information dissemination algorithm in a specialized setting. The specialized Delay Tolerant Network (DTN) system comprises static message buffers or throwboxes kept in popular places besides the mobile agents hopping from one place to another. We identify that an information dissemination technique that exploits the throwbox infrastructure can cover only a fixed number of popular places irrespective of the time spent. We notice that such DTN system has a natural bipartite network correspondence where two sets are the popular places and people visiting those places. This helps leveraging the theories of evolving bipartite networks (BNW) to provide an appropriate explanation of the observed temporal invariance of information coverage over the DTN. In this work, we first show that information coverage can be estimated by the size of the largest component in the thresholded one-mode projection of BNW. Next, we also show that exploiting a special property of BNW, the size of the largest component size can be calculated from the degree distribution. Combining these two, we derive a closed form simple equation to accurately predict the amount of information coverage in DTN which is almost impossible to achieve using the traditional techniques such as epidemic or Markov modeling. The equation shows that full coverage quickly becomes extremely difficult to achieve if the number of places increases while variation in agent's activity helps in covering more places.

==> effectofrandomness.tex <==
\section{Effect of mobility parameters}\label{sec:Randomness}

In this section, we report the study of the effect of the two
parameters related to the underlying mobility model of the agents
(as described in section \ref{sec:InformationDisseminationDTN}).

\subsection{Effect of randomness}
In general a certain randomness is involved in the place selection
strategy followed by the agents. Here we show the effect of this
randomness on the coverage achieved by the dissemination process.
In order to compare the DTN and the BNW from this perspective, we
also introduce the same randomness parameter (modeled by \rand{}
in the equation \ref{eq:pref_rand_probability}) in the BNW and use
the same procedure to calculate the probability of selecting the
next place by an agent. To study the effect of randomness in the
DTN, we first measure the time evolution of the largest connected
component of the thresholded one-mode projection in BNW as well as
the coverage in DTN for different values of \rand. Here also we
find matching pairs of \vthr{} and \buftime. Figure
~\ref{fig:RandomnessTimeSeries} shows few such sample plots for
different combinations of \nplace, \navgcon{} and \rand.

\begin{figure}
\begin{center}
\includegraphics[angle=-90,scale=0.3]{Figures/Randomness-timeSeries}
\end{center}
\caption{[Figure has to be replaced] Plot of the coverage achieved
in DTN (i.e., $G_b$) superimposed with the plot of $G_d$ in the
equivalent BNW under few different values of \rand{} for two
different combinations of \nplace{} and \navgcon. The results
shown are the average over 1000 runs of simulation.}
\label{fig:RandomnessTimeSeries}
\end{figure}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{Figures/randomness-small-mu}
\end{center}
\caption{Part (b) shows the linear-logarithmic plot of the
achieved coverage in DTN, for different values of \buftime for few
different values of \rand. Part (c) shows the size of the largest
component in the corresponding BNW (i.e., \giantbnw) for different
values of the \vthr for the same set of values of \rand. Part (a)
shows the plots of the \giantdtn{} vs \rand{} for few selected
values of \buftime{}. Part (d) shows the plots of \giantbnw{} (in
the equivalent BNW) vs \rand{} for different values of \vthr{}.
The value of \nplace{} and \navgcon{} in this example is 100 and
20, respectively. The results shown are the average over 1000 runs
of simulation.} \label{fig:effectofrandomness}
\end{figure*}


%\begin{figure}[tp]
%    \begin{minipage}[t]{0.4\linewidth}
%        %\centering
%\includegraphics[angle=0,scale=.4]{Figures/EffectOfBufferOnRandomness}
%\caption{Part (a) and (c) show the lin-log plot of the achieved
%coverage (in percentage of the number of places where the message
%is found in DTN, i.e., $G_d$) for different values of buffer time
%($b$) for few different values of randomness ($\delta$). Part (b)
%and (d) show the lin-log plot of the size of the largest component
%in the corresponding BNW (i.e., $G_b$) for different values of the
%time varying threshold ($v$) for the same set of values of
%$\delta$ (as in part (a) and (c)). The results shown are the
%average over 2000 runs of simulation.}
%        \label{fig:EffectOfBufferTime}
%    \end{minipage}
%    \hspace{0.1\linewidth}
%    \begin{minipage}[t]{0.4\linewidth}
%        %\centering
%        \includegraphics[width=1.1\textwidth]{Figures/EffectOfRandomness-1}
%        \caption{Part (a) and (c) show the plots of the stabilized value
%of the coverage (percentage of the number of places where the
%message is found in DTN, i.e., $G_d$) vs randomness ($\delta$) for
%different values of buffer time ($b$) and two different
%combinations of $N$ and $\mu$. Part (b) and (d) show the plots of
%$G_d$ (in the equivalent BNW) vs $\delta$ for different values of
%the varying threshold ($v$) under the same two combinations of $N$
%and $\mu$ as in part (a) and (c). The results shown are the
%average over 2000 runs of simulation.}
%        \label{fig:EffectOfRandomness}
%    \end{minipage}
%\end{figure}

To have a more thorough understanding we measure the achieved
coverage in the dissemination process in DTN for different values
of \buftime{} (starting from 0 to 1) and repeat the experiment for
variety of values of \rand{}. We carry out similar experiments to
study the effect of randomness on different values of the time
varying threshold values (\vthr). Figure
\ref{fig:effectofrandomness}((b), (c) show these results. It can
be observed from these results that the achieved coverage changes
noticeably for the initial values of \rand{} (between 1 and 3) and
changes very slowly for higher values. It can be also observed
that the effect of randomness is opposite in two different phases
of the refresh probability (as described in section
\ref{sec:relationshipbetweendtnandbnw}). Specifically, there
exists a refresh probability \crpd{} that depends on the value of
\nplace{} and \navgcon{} such that for \buftime $<$ \crpd, with the
increase in the value of \rand{} there is an increase in the
achieved coverage whereas for \buftime $>$ \crpd, decrease in the
achieved coverage is noticed. A similar effect can be observed in
case of BNW also. For a given value of \nplace{} and \navgcon,
there exists a varying threshold value (denoted by \crvd) below
which the effect of increase in the value of \rand{} produces
increase in the size of the largest component whereas, for \vthr
$\ge$ \crvd, an opposite effect is observed. Figure
\ref{fig:effectofrandomness}(a) and (d) show the effect of
randomness on few selected values of \buftime{} and \vthr,
respectively, for \nplace=100 and \navgcon=20, in order to further
corroborate the above observation.

\subsection{Effect of clustering exponent}
\textcolor{red}{WHERE ARE THE GRAPHS - NO GRAPHS?}
Our simulation results show that, the system is too much sensitive
with the values of $\alpha$. If we increase it, the agents tend to
move in a more clustered fashion, therefore, the number of
distinct places which get the message gets stabilized at a lower
value than that in case of $\alpha$=1 (the stabilized coverage
value decreases very fast with $\alpha$). However, if it becomes
say more than $\alpha_p$, for a given $p$ and $N$, and $\mu$, then
it does not at all stabilize. It is also noticeable that with the
increase in $\alpha$, the agent coverage gets stabilized to the
maximum achievable coverage at a faster rate. So, in a nutshell,
increase in $\alpha$ brings speed in the agent coverage but
reduces the place coverage.
%\subsection{Combined effect of overlapping life span and randomness}\label{sec:RandOvlp}
%
%We also simulate the information dissemination process in DTN when
%the life spans of the agents overlap with each other as well as
%there exists some randomness in the process of selecting the next
%place to be visited by the agents. The dotted lines in the figure
%\ref{fig:RandomnessTimeSeries} shows the coverage achieved in the
%process for overlapping life spans. It is quite clear from the
%figure that the effects of these two aspects do not interfere with
%each other. Therefore, in spite of the presence randomness in the
%place selection process by the agents, the achieved coverage after
%the system reaches the saturation point, becomes same irrespective
%of the overlapping or disjoint life spans of the agents.


==> proofOutlineSketch.tex <==
\begin{proof}
In the following we argue through an induction on number of
agents, $t$, joining the system.
 %based outline sketch,
%that the theorem holds true (with high probability). In this
%proof, by ${\mathcal G}_{P}^{*}$ we mean to say thresholded
%one-mode projection for any time varying threshold value $v$.
%Please see \cite{proofDetails} for the full details.
For $t$ = 0, ${\mathcal G}_P^{*}$ will contain $N$ isolated nodes,
and hence, the theorem is valid. We assume that for $t$ = $T$, the
theorem is true. In the following we try to show that the theorem
is still valid at $t$ = $T$ + 1, i.e., after $(T+1)^{th}$ agent
completes all its connections.

\noindent We use a result from the theory of preferentially grown
$\alpha$-BiN : \textit{The nodes which are inside the largest
component in ${\mathcal G}_P^{*}$ have strictly higher degree in
the BNW than the nodes which are outside the largest component in
${\mathcal G}_P^{*}$}. (see \cite{proofDetails} for the proof of
this result)

\noindent Let us take two subsets of nodes - $S_1$, $S_2$ where
each node in $S_1$ are inside the largest component and have
degree $u$ in the BNW while each node in $S_2$ is outside and has
degree $v$ in the BNW. Let us also take three subsets of the edges
$E_1$, $E_2$ and $E_3$, referring to the edges in between pairs of
nodes - both in $S_1$, one in $S_1$ the other in $S_2$, and both
in $S_2$, respectively. Since, with high probability most of the
$\mu$ connections created by the $(T+1)^{th}$ agent will be
towards the nodes in $S_1$ (since $u$ $>$ $v$ and preferential
connections), the rate of increment of the weights of the edges in
$E_1$, $E_2$ and $E_3$ (let us denote them by $r_1$, $r_2$ and
$r_3$) will be in the order $r_1$ $>$ $r_2$ $>$ $r_3$ (see
\cite{proofDetails} for details). This order also depicts the
order in which the edges in those subsets will become part of the
largest component (with high probability). Hence, for every value
of $t$, with high probability there will be a single largest
component in ${\mathcal G}_P^{*}$ and all other nodes will be in a
degenerate state, which proves the theorem.
\end{proof}

